FlexLoc: Conditional Neural Networks for Zero-Shot Sensor Perspective Invariance in Object Localization with Distributed Multimodal Sensors

Localization is a critical technology for various applications ranging from navigation and surveillance to assisted living. Localization systems typically fuse information from sensors viewing the scene from different perspectives to estimate the target location while also employing multiple modalities for enhanced robustness and accuracy. Recently, such systems have employed end-to-end deep neural models trained on large datasets due to their superior performance and ability to handle data from diverse sensor modalities. However, such neural models are often trained on data collected from a particular set of sensor poses (i.e., locations and orientations). During real-world deployments, slight deviations from these sensor poses can result in extreme inaccuracies. To address this challenge, we introduce FlexLoc, which employs conditional neural networks to inject node perspective information to adapt the localization pipeline. Specifically, a small subset of model weights are derived from node poses at run time, enabling accurate generalization to unseen perspectives with minimal additional overhead. Our evaluations on a multimodal, multiview indoor tracking dataset showcase that FlexLoc improves the localization accuracy by almost 50% in the zero-shot case (no calibration data available) compared to the baselines. The source code of FlexLoc is available at https://github.com/nesl/FlexLoc.

==> Contents/2_motivation.tex <==
\section{Motivation}
\label{sec:motivation}



In this section, we showcase the failure of existing multi-view object tracking models in adapting to new sensor configurations. Note that a given ``configuration'' refers to one arrangement of the three nodes. We examine both the late fusion as well as the hybrid fusion multimodal network from~\cite{wang2023gdtm}. 
The late fusion model makes independent localizations for each modality and sensor perspective, and rectifies these predictions with a Kalman Filter. In contrast, the hybrid fusion architecture promotes sharing of information between modalities and different sensor viewpoints, making one unified prediction from this compiled information. These networks do not receive any external node pose information and are evaluated in terms of generalization accuracy on new configurations after training on \emph{one single configuration}.

\xiaomin{This section is focused on evaluating single configuration models? why we need to introduce the late and early fusion approaches, which is a bit distracted.}

\subsection{Poor Generalization of Single Configuration Models}

We examine the ability of a model trained on a single configuration to adapt to different arrangements of unseen sensor positions. Table X showcases that when we evaluate both models on unseen data \emph{from the same viewpoint}, we achieve exemplary localization performance. However, both models fail when evaluated on sensor data collected from a different configuration of node viewpoints, with average distance errors of over one meter. 

The results show that a single-configuration model is unable to generalize to new configurations, as these neural networks cannot understand how sensor positions and orientations can impact object location from one single configuration. However, even if we expose the model to multiple sensor configurations during the training process to allow the network to learn spatial information from many viewpoints, the model struggles to converge and make accurate predictions (Section~\ref{sec:experiments}).


% \subsection{Multi-Configuration Models}

% We train the previous two models on X sensor configurations and evaluate them on the same set of 5 configurations, with the results shown in Table X. The poor tracking performance arises from the inability of these models to distinguish the key differences between sensor configurations. For instance, two different sensor configurations can yield images with the tracking target present at the same pixel locations with drastically different global ground truths. To accurately predict the global coordinate, the neural network must implicitly learn the difficult task of self-localizing itself within the global coordinate system from only the background content of the data. Accordingly, we postulate that providing the node pose information (position and orientation) will simplify the task and enable the neural network to learn from multi-configuration data. 

% \subsection{Local Coordinate Predictions}
% \label{subsec:localpreds}

% \emph{Ho et. al.} proposed an architecture tackling the challenge of training on multiple configurations by predicting coordinates in a given node's \emph{local coordinate system} and then applying an explicit \emph{coordinate transform matrix} to arrive at global coordinates. The intuition is that the task of predicting the car's location with respect to the \emph{node's location in a local coordinate system} is not significantly impacted by the sensor's orientation and position. Thus, by training on a large set of diverse viewpoints, the model should learn the task of local coordinate location and exhibit test time perspective invariance. While this method achieves an average localization accuracy of X cm across 5 novel viewpoints, the high tracking error renders this method incompatible with most applications. We provide a thorough comparison of \name to this method in Section X. 




